Neural Sculpting: Uncovering hierarchically modular task structure in neural networks through pruning and network analysis

Natural target functions and tasks typically exhibit hierarchical modularity -- they can be broken down into simpler sub-functions that are organized in a hierarchy. Such sub-functions have two important features: they have a distinct set of inputs (input-separability) and they are reused as inputs higher in the hierarchy (reusability). Previous studies have established that hierarchically modular neural networks, which are inherently sparse, offer benefits such as learning efficiency, generalization, multi-task learning, and transfer. However, identifying the underlying sub-functions and their hierarchical structure for a given task can be challenging. The high-level question in this work is: if we learn a task using a sufficiently deep neural network, how can we uncover the underlying hierarchy of sub-functions in that task? As a starting point, we examine the domain of Boolean functions, where it is easier to determine whether a task is hierarchically modular. We propose an approach based on iterative unit and edge pruning (during training), combined with network analysis for module detection and hierarchy inference. Finally, we demonstrate that this method can uncover the hierarchical modularity of a wide range of Boolean functions and two vision tasks based on the MNIST digits dataset.

==> Writing/Main/0_Introduction.tex <==
\section{Introduction} 

Modular tasks typically consist of smaller sub-functions that operate on distinct input modalities, such as visual, auditory, or haptic inputs. 
Additionally, modular tasks are often hierarchical, with simpler sub-functions embedded in, or reused by, more complex functions \cite{simon1991architecture}. 
Consequently, hierarchical modularity is a key organizing principle studied in both artificial and biological systems.
In neuroscience, the hierarchical modularity of the brain's neural circuits is believed to play a crucial role in its ability to process information efficiently and adaptively \cite{wagner2007road,meunier2009hierarchical,valencia2009complex,meunier2010modular}. 
This hierarchical organization allows the brain to break down complex tasks into simpler sub-tasks, which can be processed in a distributed manner.
Translating the hierarchical modularity of the brain's neural circuits to artificial neural networks (NNs) can potentially lead to more efficient, adaptable, and interpretable learning systems. 
Prior works have already shown that modular NNs efficiently adapt to new tasks \cite{veniat2020efficient, mendez2020lifelong, ostapenko2021continual} and display superior generalization over standard NNs \cite{bahdanau2018systematic,lake2018generalization,hupkes2020compositionality}.
However, those studies assume knowledge of the task's hierarchy, or hand-design, modular NNs at initialization.
Given an arbitrary task, however, we normally do not know its underlying sub-functions or their hierarchical organization.
The high-level question in this work is: if we learn a task using a NN, how can we uncover the underlying hierarchical organization of sub-functions in that task?


Recent studies have demonstrated that certain hierarchically modular structures can emerge during the training of NNs. 
Previous methods to extract those structures in NNs can be categorized into \textit{structural} and \textit{functional}. 
Structural methods organize trained networks based on the structural properties of units, such as their connectivity and edge-weights \cite{watanabe2018modular, watanabe2019interpreting, filan2021clusterability}, while functional methods consider characteristics based on unit activation \cite{hod2021detecting, lange2022clustering}. 
However, it is unclear whether the structures extracted reflect the underlying hierarchy of sub-functions in a task. 
In a recent study, Csordas et al. (\cite{csordas2020neural}) proposed a method that identifies sub-networks or modules in NNs that learn specific sub-functions.
However, this method requires knowledge of the exact sub-functions involved, and cannot be applied when such knowledge is unavailable. 
Ideally, modules corresponding to specific sub-functions should emerge through a training strategy, and a method should be available to detect these modules without explicit knowledge of the corresponding sub-functions.

Biological networks exhibit hierarchically modular structures where clusters of nodes with relatively dense internal connectivity and sparse external connectivity learn specific sub-functions \cite{valencia2009complex,meunier2010modular,clune2013evolutionary,mengistu2016evolutionary}. 
Drawing inspiration from this, we propose \textit{Neural Sculpting}, a novel approach to train and structurally organize NN units to reveal the underlying hierarchy of sub-functions in a task. 
We begin by considering sub-functions that are input-separable and reused within a hierarchically modular task. 
We show that standard training of NNs does not result in the acquisition of structural properties that reflect these sub-function properties. 
To address this, we propose an iterative unit and edge pruning method to train NNs, which results in sparse networks that do acquire those previous structural properties.
Further, we propose a method based on network analysis to uncover modules within these sparse NNs. 
Finally, we showcase the capability of the proposed methodology to reveal the structure of diverse hierarchically modular tasks.
To the best of our knowledge, this paper is the first to analyze specific sub-function properties within a hierarchically modular task and propose an end-to-end methodology to uncover its structure.
This work also sheds light on the potential of pruning and network analysis methods to uncover and harness structural properties in NNs.
\vspace{-0.2cm}
